DV-Matcher: Deformation-based Non-Rigid Point Cloud Matching Guided by Pre-trained Visual Features

In this paper, we present DV-Matcher, a novel learning-based framework for estimating dense correspondences between non-rigidly deformable point clouds. Learning directly from unstructured point clouds without meshing or manual labelling, our framework delivers high-quality dense correspondences, which is of significant practical utility in point cloud processing. Our key contributions are two-fold: First, we propose a scheme to inject prior knowledge from pre-trained vision models into geometric feature learning, which effectively complements the local nature of geometric features with global and semantic information; Second, we propose a novel deformation-based module to promote the extrinsic alignment induced by the learned correspondences, which effectively enhances the feature learning. Experimental results show that our method achieves state-of-the-art results in matching non-rigid point clouds in both near-isometric and heterogeneous shape collection as well as more realistic partial and noisy data.

==> Figs/feature_rebuttal.tex <==
\begin{figure}[b]
    \centering
    \vspace{-2em}
    \includegraphics[width=0.5\textwidth]{Figs/feature_rebuttal.png}
    \vspace{-2em}
    \caption{The arrows illustrate the entire process, with features visualized comprehensively. 2D features are visualized using PCA, while 3D shows one channel's features (left) and its map (right).}\label{fig:feature_rebuttal}
    \vspace{-1em}
\end{figure}

==> Figs/proj.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figs/proj.png}
    \vspace{-1.5em}
    \caption{Smoothing the image before (left) and after (right) to mitigate the holes. Empirically, it has minimal impact on the experimental results as reducing the rates of image holes from \textbf{40.04\%} to \textbf{0.0099\%}.}\label{fig:proj}
    \vspace{-1.5em}
\end{figure}

==> Figs/shrec16human.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Figs/shrec16human.png}
%     \vspace{-2em}
%     \caption{Qualitative results of SHREC'16 (left:cuts; right:holes).}\label{fig:shrec16human}
%     \vspace{-2em}
% \end{figure}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.5\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figs/shrec16rebuttal.png}
        \caption{Quantitative results (SHREC'16).}
        \label{fig:runtimeeffiency_left}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{Figs/runtime_accuracy_scatter.png}
        \caption{Runtime-Accuracy scatter.}
        \label{fig:runtimeeffiency_right}
    \end{subfigure}
    \vspace{-1em}
    \caption{Complementary visualizations.}
    \vspace{-2em}
    \label{fig:runtimeeffiency}
\end{figure}

==> Tabs/tab_iso.tex <==
% Please add the following required packages to your document preamble:
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t!]
    \caption{Quantitative results on SCAPE\_r, FAUST\_r and SHREC'19\_r in terms of mean geodesic errors $(\times100)$. The \textbf{best} results from the pure point cloud methods in each column are highlighted.}\label{table:iso}
    \vspace{-0.8em}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{1.9mm}
    \begin{tabular}{ccccclccc}
    \hline
    \multicolumn{1}{c}{}                                  & \textbf{Train}             & \multicolumn{3}{c}{\textbf{SCAPE\_r}}                       &  & \multicolumn{3}{c}
    {\textbf{FAUST\_r}}                       \\ \cline{3-5} \cline{7-9} 
    \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Method}}} & \textbf{Test}              & \textbf{SCAPE\_r} & \textbf{FAUST\_r} & \textbf{SHREC'19\_r} &  & \textbf{FAUST\_r} & \textbf{SCAPE\_r} & \textbf{SHREC'19\_r} \\ \hline
    3D-CODED{[}S{]}~\cite{groueix20183d}                                     &                            & 31.0              & 33.0              & \textbackslash{}    &  & 2.5               & 31.0              & \textbackslash{}    \\
    TransMatch{[}S{]}~\cite{trappolini2021shape}                                    &                            & 18.6              & 18.3              & 38.8                &  & 2.7               & 33.6              & 21.0                \\
    DiffFMaps{[}S{]}~\cite{marin2020correspondence}                                    &                            & 12.0              & 12.0              & 17.6                &  & 3.6               & 19.0              & 16.4                \\
    NIE{[}U{]}~\cite{nie}                                          &                            & 11.0              & 8.7               & 15.6                &  & 5.5               & 15.0              & 15.1                \\
    SSMSM{[}U{]}~\cite{cao2023}                                        & \multirow{-4}{*}{Trained on  Mesh}      & 4.1               & 8.5               & 7.3                 &  & 2.4               & 11.0              & 9.0                 \\ 
    DFR~\cite{dfr}  & & 2.6               & 4.0               & 5.1               &  & 3.4              &5.1             & 5.4                \\ \hline
    NDP~\cite{li2022non}                                     &                            & 16.2              & \textbackslash{}               & \textbackslash{}    &  & 20.4              & \textbackslash{}               & \textbackslash{}    \\
    AMM~\cite{amm}                                     & 
    \multirow{-1}{*}{Non-Learning}
    & 13.1             & \textbackslash{}               & \textbackslash{}    &  & 14.2              & \textbackslash{}               & \textbackslash{}    \\
    PointSetReg~\cite{zhao2024clustereg}                                    &                            & 17.1            & \textbackslash{}               & \textbackslash{}    &  & 18.3           & \textbackslash{}               & \textbackslash{}    \\
    \hline
    CorrNet3D{[}U{]}~\cite{zeng2021corrnet3d}                                     &                            & 58.0              & 63.0              & \textbackslash{}    &  & 63.0              & 58.0              & \textbackslash{}    \\
    SyNoRiM{[}S{]}~\cite{huang_multiway_2022}                                    &                            & 9.5               & 24.6              & \textbackslash{}    &  & 7.9               & 21.9              & \textbackslash{}    \\
    DPC{[}U{]}~\cite{lang2021dpc}                                           &                            & 17.3              & 11.2              & 28.7                &  & 11.1              & 17.5              & 31.0                \\
    % RMA-Net{[}U{]}~\cite{feng2021recurrent}                                      & & -             & -              & -                &  & -             & -             & -                \\
    SE-ORNet{[}U{]}~\cite{deng2023se}                                      & \multirow{-4}{*}{Learning} & 24.6              & 22.8              & 23.6                &  & 20.3              & 18.9              & 23.0                \\
    % \rowcolor[HTML]{E7E6E6} 
    % Ours-Recon.-w/o LVM                                  &                            & 13.8              & 10.4              & 14.7                &  & 8.5               & 16.1              & 15.8                \\
    % \rowcolor[HTML]{E7E6E6} 
    % Ours-Recon.                                          &                            & 7.6      & 7.3      & 9.5        &  & \textbf{4.6}      & 12.4    & 11.5      \\ 
    \rowcolor[HTML]{E7E6E6} 
    Ours[U]                                          &                            & \textbf{6.2}      & \textbf{5.1}      & \textbf{7.2}        &  & \textbf{5.4}      & \textbf{10.4}     & \textbf{9.3}       \\ \hline
    \end{tabular}
\end{table*}

==> Tabs/tab_noiso.tex <==
% Please add the following required packages to your document preamble:
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t!]
    \caption{Quantitative results on DT4D-H and SHREC'07-H in terms of mean geodesic errors $(\times100)$. The \textbf{best} results from the pure point cloud methods in each column are highlighted.}\label{table:noiso}
    \vspace{-0.8em}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{3.5mm}
    \begin{tabular}{cccclcc}
    \hline
    \multicolumn{1}{c}{}                                  & \textbf{Train}                               & \multicolumn{2}{c}{\textbf{SCAPE\_r}} &  & \multicolumn{2}{c}{\textbf{FAUST\_r}} \\ \cline{3-4} \cline{6-7} 
    \multicolumn{1}{c}{\multirow{-2}{*}{\textbf{Method}}} & \textbf{Test}                                & \textbf{DT4D-H}  & \textbf{SHREC'07-H} &  & \textbf{DT4D-H}  & \textbf{SHREC'07-H} \\ \hline
    TransMatch{[}S{]}~\cite{trappolini2021shape}                                            &                                              & 25.3             & 31.2               &  & 26.7             & 25.3               \\
    DiffFMaps{[}S{]}~\cite{marin2020correspondence}                                    &                                              & 15.9             & 15.4               &  & 18.5             & 16.8               \\
    NIE{[}U{]}~\cite{nie}                                           &                                              & 12.1             & 13.4               &  & 13.3             & 15.3               \\
    SSMSM{[}U{]}~\cite{cao2023}                                        & \multirow{-4}{*}{Trained on Mesh}                        & 8.0              & 37.7               &  & 11.8             & 42.2               \\
    \hline                          
    DPC{[}U{]}~\cite{lang2021dpc}                                           &                                              & 21.7             & 17.1               &  & 13.8             & 18.1               \\
    % RMA-Net{[}U{]}~\cite{feng2021recurrent} &                                              & -             & -              &  & -            & -              \\
    SE-ORNet{[}U{]}~\cite{deng2023se}                                     & \multirow{-2}{*}{Trained on PCD}                   & 15.5             & 27.7               &  & 12.2             & 20.9               \\
    % \rowcolor[HTML]{E7E6E6} 
    % Ours-Recon.-w/o LVM{[}U{]}                                  & \multicolumn{1}{l}{\cellcolor[HTML]{E7E6E6}} & 10.3             & 14.3               &  & 11.2             & 16.4               \\
    % \rowcolor[HTML]{E7E6E6} 
    % Ours-Recon.{[}U{]}                                          & \multicolumn{1}{l}{\cellcolor[HTML]{E7E6E6}} & 7.7     & 8.9       &  & 9.0     & 8.9       \\ 
    \rowcolor[HTML]{E7E6E6} 
    Ours{[}U{]}                                          & \multicolumn{1}{l}{\cellcolor[HTML]{E7E6E6}} & \textbf{6.9}     & \textbf{7.7}       &  & \textbf{8.1}     & \textbf{8.2}       \\
    \hline
    \end{tabular}
\end{table*}

==> Tabs/tab_rebuttal.tex <==
% Please add the following required packages to your document preamble:
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[H]
    \caption{Train on SCAPE\_r and test on SCAPE\_r, which shows the improvement of our projection after the non-linear color is assigned.
    }\label{table:rebuttal}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{3mm}
    \vspace{1em} % 增加垂直间距
    \begin{tabular}{ccc}
    \hline
                               & \textbf{un-colored} & \textbf{colored} \\
    \hline
    \textbf{Geo. error (×100)} & 9.0                 & \textbf{7.6}             \\ \hline
                               &                     &    
    \end{tabular}
\end{table}

==> Tabs/tab_topkids.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Mean geodesic errors on dataset with topological noise.}\label{table:topkids}
\vspace{-1em}
\centering
\footnotesize
\begin{tabular}{lccc
>{\columncolor[HTML]{E7E6E6}}c }
\hline
Train\textbackslash{}Test & PointSetReg & DPC  & SE-ORNet & Ours          \\ \hline
SCAPE\_r\textbackslash{}TOPKIDS & 20.3        & 20.9 & 20.2     & \textbf{12.9} \\ \hline
\end{tabular}
\vspace{-2em}
\end{table}
